Lower Bounds for the Complexity of Monadic Second-Order Logic

Courcelle's famous theorem from 1990 states that any property of graphs definable in monadic second-order logic (MSO) can be decided in linear time on any class of graphs of bounded treewidth, or in other words, MSO is fixed-parameter tractable in linear time on any such class of graphs. From a logical perspective, Courcelle's theorem establishes a sufficient condition, or an upper bound, for tractability of MSO-model checking. Whereas such upper bounds on the complexity of logics have received significant attention in the literature, almost nothing is known about corresponding lower bounds. In this paper we establish a strong lower bound for the complexity of monadic second-order logic. In particular, we show that if C is any class of graphs which is closed under taking subgraphs and whose treewidth is not bounded by a polylogarithmic function (in fact, $\log^c n$ for some small c suffices) then MSO-model checking is intractable on C (under a suitable assumption from complexity theory).

==> conclusion.tex <==

\Section{Conclusion}
\label{sec:conclusion}

We have presented a strong intractability result for $\MSO$ on graph
classes of unbounded treewidth. In comparison to Courcelle's theorem,
Courcelle's theorem requires the treewidth to be constant whereas our
result refers to classes whose treewidth is essentially not bounded
logarithmically. As the examples in \cite{MakowskyMarino03} show, there
are classes of graphs of unbounded treewidth, closed under subgraphs,
which admit tractable $\MSO$-model-checking. On the other hand, this
is very unlikely to be the case for all classes of logarithmic
treewidth. Exploring tractability and intractability of $\MSO$ on
classes of unbounded treewidth, but bounded by $\log n$, might lead
to interesting new results on the boundary of $\MSO$-tractability.

The results reported in this part of the thesis refer to $\MSO$,
i.e.~MSO with quantification over sets of edges. For MSO without edge
set quantification, referred to as $\gMSO_1$, it can be shown that
$\gMSO_1$ is tractable on any class $\CCC$ of graphs of bounded
\emph{cliquewidth}. Again, except for the examples in
\cite{MakowskyMarino03}, not much is known about $\gMSO_1$ and graph
classes of unbounded cliquewidth and it would be very interesting to
establish similar results as in this work for the case of
cliquewidth. This, however, is much more difficult as no good
obstruction similar to grid-like minors is known for this case.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "lics10"
%%% End: 

